MusicHiFi: Fast High-Fidelity Stereo Vocoding

Diffusion-based audio and music generation models commonly perform generation by constructing an image representation of audio (e.g., a mel-spectrogram) and then convert it to audio using a phase reconstruction model or vocoder. Typical vocoders, however, produce monophonic audio at lower resolutions (e.g., 16-24 kHz), which limits their usefulness. We propose MusicHiFi -- an efficient high-fidelity stereophonic vocoder. Our method employs a cascade of three generative adversarial networks (GANs) that convert low-resolution mel-spectrograms to audio, upsamples to high-resolution audio via bandwidth extension, and upmixes to stereophonic audio. Compared to past work, we propose 1) a unified GAN-based generator and discriminator architecture and training procedure for each stage of our cascade, 2) a new fast, near downsampling-compatible bandwidth extension module, and 3) a new fast downmix-compatible mono-to-stereo upmixer that ensures the preservation of monophonic content in the output. We evaluate our approach using objective and subjective listening tests and find our approach yields comparable or better audio quality, better spatialization control, and significantly faster inference speed compared to past work. Sound examples are at \url{https://MusicHiFi.github.io/web/}.

==> SPL.tex <==
\section{SPL submission questions}
Please consult the journal’s \href{https://ieeexplore.ieee.org/xpl/aboutJournal.jsp?punumber=97}{Aims and Scope} for more detail on topics that are considered to fall within the scope of the journal.

The appropriate length of the response is a couple of sentences. The absence of a suitable response may be taken into account when making a decision in cases of possible immediate rejection for reasons of scope.

\subsection{If the manuscript has more than one author, briefly describe every author’s significant intellectual contribution (max 25 words per author). }

Ge Zhu implemented all major functionality of the work, developed critical ideas for the BWE, ran all experiments and evaluation, wrote the paper, and webpage.

Juan-Pablo Caceres was co-lead mentor on research ideas and evaluation and edited the paper.

Zhiyao Duan contributed research ideas for bandwidth expansion and listening studies and edited the paper.

Nicholas J. Bryan was co-lead mentor throughout, code for the listening test, dataloaders, distributed compute, significance tests, and led paper editing and demo video.



\subsection{What is the contribution of this paper, within the scope of IEEE Signal Processing Letters?}

We contribute MusicHiFi, a new efficient high-fidelity stereophonic vocoder. Our method employs a GAN-triplet cascade that converts low-resolution single-channel mel-spectrograms (e.g., 22.05 kHz) to stereo high-resolution waveforms (e.g., stereo 44.1 kHz) leveraging vocoder, BWE, and M2S modules. Our method can be seamlessly integrated into low-sampling rate mel-spectrograms music generators, used to enhance the fidelity of a low-resolution audio recording, and/or used to spatialize monophonic music. We evaluate our approach via multiple objective and subjective listening tests and find our approach yields equal or better vocoding, BWE, and M2S quality with significantly faster inference speed. Our contributions include: 1) A unified GAN-based generator, discriminator, and training recipe for vocoding, BWE, and M2S upmixing to simplif development, 2) A new efficient bandwidth extension method that maintains the low-frequency content in upsampled audio through skip connections, and 3) A novel mono-to-stereo method that uses a middle-side stereo encoding that fully preserves monophonic content and offers superior spatialization width control.


\subsection{Why is the contribution significant (What impact will it have)?}

The focus of our work was to develop a single unified deep learning ``recipe'' to address three foundational signal processing problems including vocoding, bandwidth expansion (BWE), and mono-to-stereo upmixing (M2S). All three such tasks are useful for audio and music signal enhancement as well as the rapidly developing field of music generation. When compared to several baselines for each of the three tasks, we show how our unified approach yields several benefits including a comparable or improved vocoding and BWE and improve M2S quality, improved M2S controllability, and dramatically faster GPU inference speed.


\subsection{What are the three papers in the published literature most closely related to this paper? Please provide full citation details, including DOI references where possible.}

1) S.-g. Lee, W. Ping, B. Ginsburg, B. Catanzaro, and S. Yoon. ``BigVGAN: A universal neural vocoder with large-scale training.'' International Conference on Learning Representations (ICLR), 2023. https://arxiv.org/abs/2206.04658 (2022).

2) R. Kumar, P. Seetharaman, A. Luebs, I. Kumar, K. Kumar. ``High-Fidelity Audio Compression with Improved RVQGAN.'' Neural Information Processing Systems (NeurIPS), 2023.

3) M. Mandel, O. Tal, Y. Adi, ``AERO: Audio super resolution in the spectral domain''. IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP), 2023.

\subsection{What is distinctive/new about the current paper relative to these previously published works?}

Our proposed work is distinctive because we use a single single GAN generator, discriminator, and training recipe to address three critical signal processing applications. Each application is useful by itself, but also useful together in sequence when used for music generation applications. Furthermore, our combined method is very fast and dramatically faster than alternative methods for bandwidth expansion and mono-to-stereo upmixing. 

==> table/cascaded_table.tex <==
\begin{table}[!t]
\caption{Cascaded system overall performance for our proposed MusicHiFi}
\label{tab:aqa}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc|cc}
\toprule
\multirow{2}{*}{\textbf{Stage}}&\multicolumn{2}{c}{FMA-small} & \multicolumn{2}{c}{DSD100-test} \\
\cline{2-5}\specialrule{0em}{1pt}{1pt}
\multicolumn{1}{c}{} &\textbf{ViSQOL}($\uparrow$) & \textbf{RTF}($\uparrow$) & \textbf{ViSQOL}($\uparrow$) & \textbf{RTF}($\uparrow$)\\
\hline 
BigVGAN+Aero+DSP& 4.67& - & 4.67 & - \\
AudioSR+DSP& 4.22 &- & 4.14 & - \\
Ours& 4.17&-& 4.10    &-\\
\bottomrule
\end{tabular}
}
\end{table}

==> table/main_table.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of objective metrics}
\scriptsize
\begin{tabular}{cccccccc}
\toprule
\textbf{Dataset} & \textbf{Stage} &\textbf{Method} &Mel-distance ($\downarrow$)& STFT-distance ($\downarrow$) & ViSQOL($\uparrow$) & SI-SDR($\uparrow$) & Real Time Factor($\uparrow$) \\
\midrule
\multirow{10}{*}{In-house} &\multirow{4}{*}{Vocoding}&HiFi-GAN& 1.05 & 0.61 &4.52& \textbf{21.24}&-  \\
&&HiFi-GAN-large&1.01& 0.54&4.55  &20.85 &-  \\
&& BigVGAN& 0.91 & 0.39 &4.63&20.27 &-\\
&&MusicHiFi-V& \textbf{0.85} & \textbf{0.33} &\textbf{4.67}& 21.16&- \\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&\multirow{2}{*}{Bandwidth Extension}&Aero~\cite{mandel2023aero}& 0.06/1.23/0.55 & 0.03/0.57/0.13 &\textbf{4.24}& -&-\\
&&MusicHiFi-BWE& 0.09/1.30/0.60 & 0.02/0.61/0.12 &4.22& -&- \\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&\multirow{2}{*}{Mono-to-stereo}&DSP~\cite{michael2019s3a}& 1.18/1.19/0.17/2.38 & 0.97/0.97/0.15/2.16 &4.69& -&- \\
&&MusicHiFi-M2S& 0.93/0.93/0.00/1.57 & 0.72/0.72/0.00/1.39 &\textbf{4.73}& -&- \\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&Cascaded&MusicHiFi& - & - &4.17& -&- \\
\midrule
% \multirow{8}{*}{FMA-subset}&\multirow{4}{*}{Vocoding}  &HiFi-GAN-base& 1.09 & 0.64 &4.52& \textbf{32.45}&-  \\
% &&HiFi-GAN-large&1.04&0.57&4.56&31.89&-\\
% && BigVGAN-base&0.94&0.41&4.62&30.01&-\\
% &&BigGAN-DAC-base& \textbf{0.87}&\textbf{0.35}&\textbf{4.67}&31.57&-\\
% % &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
% \cmidrule(lr){2-8}
% &\multirow{2}{*}{Bandwidth Extension}&Aero& 0.07/1.60/0.89 & 0.03/0.73/0.24 &\textbf{4.12}& -&-\\
% &&BigGAN-DAC-base&0.09/1.76/1.01& 0.02/0.79/0.26 &4.08& -&-\\
% % &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
% \cmidrule(lr){2-8}
% &\multirow{2}{*}{Mono-to-stereo}&DSP&1.18/1.18/0.99/2.29 & 1.10/1.11/1.08/2.16 &4.70& -&-\\
% &&BigGAN-DAC-base& 0.80/0.81/0.00/2.03 & 0.62/0.62/0.00/1.88 &4.73& -&-\\
% % &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
% \cmidrule(lr){2-8}
% &Cascaded&BigGAN-DAC-base& - & - &4.03& -&- \\
% \midrule
\multirow{11}{*}{DSD100-test}&\multirow{4}{*}{Vocoding}&HiFi-GAN& 1.09 & 0.65&4.47&28.62\\
&&HiFi-GAN-large&1.06&0.60&4.48&\textbf{30.29}&-\\
&& BigVGAN&0.94&0.41&4.61&27.75& -\\
&&MusicHiFi-V& \textbf{0.87}&\textbf{0.33}&\textbf{4.67}&28.49\\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&\multirow{3}{*}{Bandwidth Extension}&Aero~\cite{mandel2023aero}& 0.05/1.16/0.51	&0.02/0.54/0.12 &\textbf{4.18}&-\\
&&AudioSR~\cite{liu2023audiosr}& 0.64/2.25/1.23* & 0.36/1.68/0.51* &-& -&-\\
&&MusicHiFi-BWE& 0.08/1.18/0.55&0.02/0.56/0.11&4.14\\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&\multirow{2}{*}{Mono-to-stereo}&DSP~\cite{michael2019s3a}& 1.26/1.25/1.07/1.87	&1.14/1.14/1.09/1.70 &4.69& -&-\\
&&MusicHiFi-M2S& 0.90/0.90/0.00/1.70&0.71/0.70/0.00/1.53 &\textbf{4.73}& -&-\\
% &BigGAN-DAC-2048& & 3.66 & 2.51 &3.70& 1.99&9.52 & 1.39  &5.95 & 1.51 & 0.51 \\
\cmidrule(lr){2-8}
&Cascaded&MusicHiFi& - & - &4.10& -&- \\
\bottomrule
\end{tabular}

\label{tab:music_sep_results}
\end{table*}

==> table/mushra.tex <==
\begin{table}[!t]
\caption{System configurations for MUSHRA test. 
Upper table represents the BWE subjective test and lower represents the evaluation for M2S.}
\label{tab:mushra}
\centering
\scriptsize
% \resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline 
Group Name&Vocoder & BWE & M2S\\
\hline 
(a)& \multicolumn{2}{c|}{AudioSR}& -\\
\cline{2-4}
(b)& MusicHiFi-V&Aero & -\\
\cline{2-4}
(b)&\multicolumn{2}{c|}{MusicHiFi-Mono}  & - \\ 
\hline 
(d) &\multicolumn{2}{c|}{MusicHiFi-Mono} & DSP \\
\cline{2-4}
(e)& \multicolumn{3}{c}{MusicHiFi}\\
\cline{2-4}

\hline 
\end{tabular}

\end{table}
